Inference for Dependent Data with Learned Clusters

This paper presents and analyzes an approach to cluster-based inference for dependent data. The primary setting considered here is with spatially indexed data in which the dependence structure of observed random variables is characterized by a known, observed dissimilarity measure over spatial indices. Observations are partitioned into clusters with the use of an unsupervised clustering algorithm applied to the dissimilarity measure. Once the partition into clusters is learned, a cluster-based inference procedure is applied to a statistical hypothesis testing procedure. The procedure proposed in the paper allows the number of clusters to depend on the data, which gives researchers a principled method for choosing an appropriate clustering level. The paper gives conditions under which the proposed procedure asymptotically attains correct size. A simulation study shows that the proposed procedure attains near nominal size in finite samples in a variety of statistical testing problems with dependent data.

==> table_summary_iv_baseline_large_stretch.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: IV - BASELINE ($N_{\mathrm{pan}}=820$)}
\label{table_summary_iv_baseline_large}
	\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
			Method & Estim. Median & Estim. MAD & Size & \multicolumn{4}{c}{Power}\\
			\cline{5-8}
			& & & & -1 & -0.5 & 0.5 & 1\\
			\hline
			SK     & 0.004  & 0.089 & 0.390 & 1.000 & 1.000 & 0.973 & 1.000 \\
			UNIT-U & 0.004  & 0.089 & 0.700 & 1.000 & 0.995 & 1.000 & 1.000 \\
			UNIT   & 0.004  & 0.089 & 0.048 & 0.998 & 0.870 & 1.000 & 1.000 \\
			CCE    & 0.004  & 0.089 & 0.051 & 0.989 & 0.837 & 0.963 & 1.000 \\
			IM     & -0.041 & 0.061 & 0.055 & 0.994 & 0.940 & 0.998 & 0.999 \\
			CRS    & -0.042 & 0.061 & 0.056 & 0.999 & 0.999 & 0.930 & 0.993\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated median, estimated MAD, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> table_summary_iv_baseline_small_stretch.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: IV - BASELINE ($N_{\mathrm{pan}}=205$)}
\label{table_summary_iv_baseline}
	\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Median & Estim. MAD & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
SK     & 0.002  & 0.114 & 0.362 & 1.000 & 0.999 & 0.913 & 0.993 \\
UNIT-U & 0.002  & 0.114 & 0.568 & 0.996 & 0.950 & 1.000 & 1.000 \\
UNIT   & 0.002  & 0.114 & 0.074 & 0.954 & 0.711 & 0.910 & 1.000 \\
CCE    & 0.002  & 0.114 & 0.062 & 0.927 & 0.652 & 0.729 & 0.987 \\
IM     & -0.059 & 0.091 & 0.046 & 0.930 & 0.736 & 0.951 & 0.985 \\
CRS    & -0.061 & 0.095 & 0.040 & 0.992 & 0.992 & 0.680 & 0.921\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated median, estimated MAD, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> table_summary_iv_sar_large_stretch.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: IV - SAR ($N_{\mathrm{pan}}=820$)}
	\label{table_summary_iv_sar_large}
		\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Median & Estim. MAD & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
SK     & 0.003  & 0.076 & 0.144 & 1.000 & 1.000 & 0.953 & 0.997 \\
UNIT-U & 0.003  & 0.076 & 0.389 & 1.000 & 0.983 & 1.000 & 1.000 \\
UNIT   & 0.003  & 0.076 & 0.118 & 0.998 & 0.948 & 1.000 & 1.000 \\
CCE    & 0.003  & 0.076 & 0.030 & 0.979 & 0.804 & 0.898 & 0.999 \\
IM     & -0.052 & 0.130 & 0.022 & 0.774 & 0.561 & 0.756 & 0.864 \\
CRS    & -0.052 & 0.123 & 0.037 & 0.921 & 0.891 & 0.652 & 0.847\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated median, estimated MAD, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_alphaHat_distr.tex <==

\begin{table}[t]
	\caption{Distribution of $\hat\alpha$}
    \label{tab: hat alpha}
	\centering
	\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}	
		\begin{tabular}{m{.1\textwidth} >{\centering}m{.1\textwidth} >{\centering}m{.1\textwidth} >{\centering}m{.1\textwidth} >{\centering}m{.1\textwidth} >{\centering\arraybackslash}m{.1\textwidth}}
			\hline
			\hline
			& \multicolumn{5}{c}{Quantile}            \\
			\cline{2-6}
			& 0.1  & 0.25   & 0.5    & 0.75   & 0.9    \\
			\hline
			\multicolumn{6}{c}{A. OLS - BASELINE} \\
			\hline
			CCE                  & 0.004          & 0.006 & 0.008 & 0.010 & 0.012 \\
			IM                   & 0.039          & 0.042 & 0.046 & 0.050 & 0.050 \\
			CRS                  & 0.039          & 0.043 & 0.047 & 0.050 & 0.050 \\
			\hline
			\multicolumn{6}{c}{B. OLS - SAR}\\
			\hline
			CCE                  & 0.021          & 0.024 & 0.027 & 0.031 & 0.034 \\
			IM                   & 0.047          & 0.049 & 0.050 & 0.050 & 0.050 \\
			CRS                  & 0.047          & 0.047 & 0.050 & 0.050 & 0.050 \\
			\hline
			\multicolumn{6}{c}{C. IV - BASELINE}\\
			\hline
			CCE                  & 0.004          & 0.005 & 0.007 & 0.008 & 0.010 \\
			IM                   & 0.045          & 0.048 & 0.050 & 0.050 & 0.050 \\
			CRS                  & 0.039          & 0.039 & 0.047 & 0.050 & 0.050 \\
			\hline
			\multicolumn{6}{c}{D. IV - SAR}\\
			\hline
			CCE                  & 0.014          & 0.020 & 0.025 & 0.029 & 0.033 \\
			IM                   & 0.032          & 0.050 & 0.050 & 0.050 & 0.050 \\
			CRS                  & 0.008          & 0.043 & 0.050 & 0.050 & 0.050\\
			\hline
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for $\hat \alpha$, the data-dependent p-value threshold for rejecting a hypothesis at the 5\% level obtained in \eqref{eq: optimization problem}. Panels correspond to the different designs described in Section \ref{subsec: DGP}. For each design and DGP we report the .1, .25, .5, .75, and .9 quantiles of the simulation distribution of $\hat\alpha$. 
		\end{tablenotes}
	\end{threeparttable}
\end{table}


==> tables/table_kHat_distr.tex <==
\begin{table}[t]
	\caption{Distribution of $\hat\G$}
	\label{tab: hat k}
	\centering
	\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}	
		\begin{tabular}{m{.1\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} >{\centering\arraybackslash}m{.08\textwidth}}%{cccccccc}
			\hline
			\hline
			& $\hat \G=2$ & 3 & 4 & 5 & 6 & 7 & 8 \\
			\hline
\multicolumn{8}{c}{A. OLS - BASELINE}\\
\hline
CCE                  & 0.000          & 0.000 & 0.001 & 0.098 & 0.311 & 0.260 & 0.330 \\
IM                   & 0.000          & 0.000 & 0.000 & 0.007 & 0.018 & 0.113 & 0.862 \\
CRS                  & 0.000          & 0.000 & 0.000 & 0.000 & 0.001 & 0.099 & 0.900 \\
\hline
\multicolumn{8}{c}{B. OLS - SAR}\\
\hline
CCE                  & 0.000          & 0.001 & 0.022 & 0.051 & 0.113 & 0.268 & 0.545 \\
IM                   & 0.000          & 0.003 & 0.069 & 0.554 & 0.040 & 0.176 & 0.158 \\
CRS                  & 0.000          & 0.000 & 0.000 & 0.000 & 0.001 & 0.401 & 0.598 \\
\hline
\multicolumn{8}{c}{C. IV - BASELINE}\\
\hline
CCE                  & 0.000          & 0.001 & 0.001 & 0.039 & 0.242 & 0.261 & 0.456 \\
IM                   & 0.000          & 0.000 & 0.005 & 0.051 & 0.062 & 0.066 & 0.816 \\
CRS                  & 0.000          & 0.000 & 0.000 & 0.000 & 0.000 & 0.157 & 0.843 \\
\hline
\multicolumn{8}{c}{D. IV - SAR}\\
\hline
CCE                  & 0.006          & 0.027 & 0.048 & 0.047 & 0.071 & 0.257 & 0.544 \\
IM                   & 0.005          & 0.078 & 0.240 & 0.568 & 0.030 & 0.038 & 0.041 \\
CRS                  & 0.000          & 0.000 & 0.000 & 0.000 & 0.032 & 0.480 & 0.488\\
			\hline
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for $\hat \G$, the data-dependent number of clusters obtained in \eqref{eq: optimization problem}. Panels correspond to the different designs described in Section \ref{subsec: DGP}. Each entry reports the simulation probability of $\hat \G$ being equal to the value given in the column label for the procedure indicated in the row label. 
		\end{tablenotes}
	\end{threeparttable}
\end{table}

==> tables/table_simulation_results.tex <==

\begin{table}[t]
	\centering
	\renewcommand{\arraystretch}{1.5}
	\caption{Simulation Results}
	\label{table_summary}
	\begin{threeparttable}	
		\begin{tabular}{m{.1\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} m{.1\textwidth} >{\centering}m{.08\textwidth} >{\centering}m{.08\textwidth} >{\centering\arraybackslash}m{.08\textwidth}}%{lccccccc}
			\hline
			\hline
			& \multicolumn{3}{c}{OLS} & & \multicolumn{3}{c}{IV} \\
			\cline{2-4} \cline{6-8}
			Method & Bias & RMSE & Size &  & Median Bias & MAD & Size \\
			\hline
\multicolumn{8}{c}{A. BASELINE}\\
\hline
SK          & \multirow{4}{*}{0.015}  & \multirow{4}{*}{0.337} & 0.381 &  & \multirow{4}{*}{0.002}  & \multirow{4}{*}{0.114} & 0.362 \\
UNIT-U      &        &       & 0.577 &  &        &       & 0.568 \\
UNIT        &        &       & 0.047 &  &        &       & 0.074 \\
CCE         &        &       & 0.046 &  &        &       & 0.062 \\
IM          & 0.014  & 0.213 & 0.044 &  & -0.059 & 0.091 & 0.046 \\
CRS         & 0.014  & 0.213 & 0.042 &  & -0.061 & 0.095 & 0.040 \\
\hline
\multicolumn{8}{c}{B. SAR}\\
\hline
SK          & \multirow{4}{*}{-0.013} & \multirow{4}{*}{0.866} & 0.447 &  & \multirow{4}{*}{0.002}  & \multirow{4}{*}{0.280} & 0.324 \\
UNIT-U      &        &       & 0.639 &  &        &       & 0.502 \\
UNIT        &        &       & 0.359 &  &        &       & 0.256 \\
CCE         &        &       & 0.047 &  &        &       & 0.083 \\
IM          & -0.006 & 0.385 & 0.038 &  & -0.046 & 0.158 & 0.025 \\
CRS         & -0.003 & 0.354 & 0.049 &  & -0.095 & 0.213 & 0.041\\
			\hline 			
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Results from the OLS Simulation (in columns labeled ``OLS'') and IV Simulation (in columns labeled ``IV'') described in Section \ref{subsec: DGP}. Row labels indicate inferential method. Panel A corresponds to the {BASELINE} design where tuning parameters for UNIT, CCE, IM, and CRS are selected based on calculating size and power from feasible estimates of a correctly specific parametric model. Panel B corresponds to the {SAR} design where tuning parameters for UNIT, CCE, IM, and CRS are selected based on calculating size and power from feasible estimates of a misspecified parametric model. For the OLS designs, we report the bias and RMSE of the point estimator associated with each procedure along with size of 5\% level tests. For the IV designs, we report the median bias and MAD of the point estimator associated with each procedure along with size of 5\% level tests.
		\end{tablenotes}
	\end{threeparttable}
\end{table}

==> tables/table_summary_iv_baseline_large.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: IV - BASELINE ($N_{\mathrm{pan}}=820$)}
\label{table_summary_iv_baseline_large}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
			Method & Estim. Median & Estim. MAD & Size & \multicolumn{4}{c}{Power}\\
			\cline{5-8}
			& & & & -1 & -0.5 & 0.5 & 1\\
			\hline
			SK     & 0.004  & 0.089 & 0.390 & 1.000 & 1.000 & 0.973 & 1.000 \\
			UNIT-U & 0.004  & 0.089 & 0.700 & 1.000 & 0.995 & 1.000 & 1.000 \\
			UNIT   & 0.004  & 0.089 & 0.048 & 0.998 & 0.870 & 1.000 & 1.000 \\
			CCE    & 0.004  & 0.089 & 0.051 & 0.989 & 0.837 & 0.963 & 1.000 \\
			IM     & -0.041 & 0.061 & 0.055 & 0.994 & 0.940 & 0.998 & 0.999 \\
			CRS    & -0.042 & 0.061 & 0.056 & 0.999 & 0.999 & 0.930 & 0.993\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated median, estimated MAD, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_summary_iv_baseline_small.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: IV - BASELINE ($N_{\mathrm{pan}}=205$)}
\label{table_summary_iv_baseline}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Median & Estim. MAD & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
SK     & 0.002  & 0.114 & 0.362 & 1.000 & 0.999 & 0.913 & 0.993 \\
UNIT-U & 0.002  & 0.114 & 0.568 & 0.996 & 0.950 & 1.000 & 1.000 \\
UNIT   & 0.002  & 0.114 & 0.074 & 0.954 & 0.711 & 0.910 & 1.000 \\
CCE    & 0.002  & 0.114 & 0.062 & 0.927 & 0.652 & 0.729 & 0.987 \\
IM     & -0.059 & 0.091 & 0.046 & 0.930 & 0.736 & 0.951 & 0.985 \\
CRS    & -0.061 & 0.095 & 0.040 & 0.992 & 0.992 & 0.680 & 0.921\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated median, estimated MAD, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_summary_iv_sar_large.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: IV - SAR ($N_{\mathrm{pan}}=820$)}
	\label{table_summary_iv_sar_large}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Median & Estim. MAD & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
SK     & 0.003  & 0.076 & 0.144 & 1.000 & 1.000 & 0.953 & 0.997 \\
UNIT-U & 0.003  & 0.076 & 0.389 & 1.000 & 0.983 & 1.000 & 1.000 \\
UNIT   & 0.003  & 0.076 & 0.118 & 0.998 & 0.948 & 1.000 & 1.000 \\
CCE    & 0.003  & 0.076 & 0.030 & 0.979 & 0.804 & 0.898 & 0.999 \\
IM     & -0.052 & 0.130 & 0.022 & 0.774 & 0.561 & 0.756 & 0.864 \\
CRS    & -0.052 & 0.123 & 0.037 & 0.921 & 0.891 & 0.652 & 0.847\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated median, estimated MAD, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_summary_iv_sar_small.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: IV - SAR ($N_{\mathrm{pan}}=205$)}
	\label{table_summary_iv_sar}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Median & Estim. MAD & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
SK     & 0.002  & 0.280 & 0.324 & 0.898 & 0.655 & 0.627 & 0.768 \\
UNIT-U & 0.002  & 0.280 & 0.502 & 0.797 & 0.675 & 0.798 & 0.942 \\
UNIT   & 0.002  & 0.280 & 0.256 & 0.737 & 0.604 & 0.567 & 0.839 \\
CCE    & 0.002  & 0.280 & 0.083 & 0.634 & 0.464 & 0.282 & 0.626 \\
IM     & -0.046 & 0.158 & 0.025 & 0.658 & 0.420 & 0.470 & 0.773 \\
CRS    & -0.095 & 0.213 & 0.041 & 0.778 & 0.703 & 0.331 & 0.563\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated median, estimated MAD, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_summary_ols_baseline_large.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: OLS - BASELINE ($N_{\mathrm{pan}}=820$)}
	\label{table_summary_ols_baseline_large}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Mean & Estim. RMSE & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
 SK     & 0.002  & 0.259 & 0.395 & 0.998 & 0.856 & 0.847 & 0.998 \\
 UNIT-U & 0.002  & 0.259 & 0.700 & 1.000 & 0.938 & 0.944 & 1.000 \\
 UNIT   & 0.002  & 0.259 & 0.039 & 0.962 & 0.517 & 0.496 & 0.960 \\
 CCE    & 0.002  & 0.259 & 0.052 & 0.917 & 0.449 & 0.449 & 0.899 \\
 IM     & -0.001 & 0.146 & 0.058 & 1.000 & 0.877 & 0.881 & 1.000 \\
 CRS    & -0.001 & 0.146 & 0.058 & 1.000 & 0.871 & 0.868 & 1.000\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated mean, estimated RMSE, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_summary_ols_baseline_small.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: OLS - BASELINE ($N_{\mathrm{pan}}=205$)}
	\label{table_summary_ols_baseline}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Mean & Estim. RMSE & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
SK     & 0.015 & 0.337 & 0.381 & 0.974 & 0.730 & 0.727 & 0.981 \\
UNIT-U & 0.015 & 0.337 & 0.577 & 0.992 & 0.844 & 0.832 & 0.987 \\
UNIT   & 0.015 & 0.337 & 0.047 & 0.831 & 0.335 & 0.319 & 0.818 \\
CCE    & 0.015 & 0.337 & 0.046 & 0.717 & 0.292 & 0.248 & 0.704 \\
IM     & 0.014 & 0.213 & 0.044 & 0.979 & 0.553 & 0.523 & 0.962 \\
CRS    & 0.014 & 0.213 & 0.042 & 0.957 & 0.514 & 0.519 & 0.970\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated mean, estimated RMSE, size, and power against four alternatives (-1, -0.5, 0.5, 1). 
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_summary_ols_sar_large.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: OLS- SAR ($N_{\mathrm{pan}}=820$)}
	\label{table_summary_ols_sar_large}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Mean & Estim. RMSE & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
 SK     & 0.003  & 0.229 & 0.154 & 0.996 & 0.780 & 0.787 & 0.990 \\
 UNIT-U & 0.003  & 0.229 & 0.405 & 0.999 & 0.909 & 0.903 & 1.000 \\
 UNIT   & 0.003  & 0.229 & 0.123 & 0.992 & 0.756 & 0.743 & 0.995 \\
 CCE    & 0.003  & 0.229 & 0.020 & 0.860 & 0.363 & 0.364 & 0.848 \\
 IM     & -0.013 & 0.249 & 0.035 & 0.908 & 0.465 & 0.524 & 0.911 \\
 CRS    & -0.013 & 0.229 & 0.062 & 0.959 & 0.612 & 0.553 & 0.938\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated mean, estimated RMSE, size, and power against four alternatives (-1, -0.5, 0.5, 1).
		\end{tablenotes}
	\end{threeparttable}
\end{table}



==> tables/table_summary_ols_sar_small.tex <==




\begin{table}[H]
	\centering
	\renewcommand{\arraystretch}{1.2}
	\caption{Summary: OLS- SAR ($N_{\mathrm{pan}}=205$)}
	\label{table_summary_ols_sar}
	\begin{threeparttable}	
		\begin{tabular}{cccccccccccccc}
			\hline
			\hline
Method & Estim. Mean & Estim. RMSE & Size & \multicolumn{4}{c}{Power}\\
 \cline{5-8}
 & & & & -1 & -0.5 & 0.5 & 1\\
 \hline
SK     & -0.013 & 0.866 & 0.447 & 0.688 & 0.514 & 0.517 & 0.691 \\
UNIT-U & -0.013 & 0.866 & 0.639 & 0.761 & 0.683 & 0.681 & 0.766 \\
UNIT   & -0.013 & 0.866 & 0.359 & 0.657 & 0.461 & 0.452 & 0.656 \\
CCE    & -0.013 & 0.866 & 0.047 & 0.362 & 0.160 & 0.167 & 0.372 \\
IM     & -0.006 & 0.385 & 0.038 & 0.586 & 0.216 & 0.189 & 0.588 \\
CRS    & -0.003 & 0.354 & 0.049 & 0.674 & 0.231 & 0.256 & 0.670\\
 \hline 
		\end{tabular}
		\begin{tablenotes}
			\item Notes: Simulation results for estimation in the design described in Section \ref{simulation}. 
			The nominal size is 0.05. 
			Estimates are presented for the estimators, SK, UNIT-U, UNIT, CCE, IM, CRS described in the text. 
			Columns display method, estimated mean, estimated RMSE, size, and power against four alternatives (-1, -0.5, 0.5, 1).
		\end{tablenotes}
	\end{threeparttable}
\end{table}


